Dispelling the Mirage of Progress in Offline MARL through Standardised Baselines and Evaluation

Offline multi-agent reinforcement learning (MARL) is an emerging field with great promise for real-world applications. Unfortunately, the current state of research in offline MARL is plagued by inconsistencies in baselines and evaluation protocols, which ultimately makes it difficult to accurately assess progress, trust newly proposed innovations, and allow researchers to easily build upon prior work. In this paper, we firstly identify significant shortcomings in existing methodologies for measuring the performance of novel algorithms through a representative study of published offline MARL work. Secondly, by directly comparing to this prior work, we demonstrate that simple, well-implemented baselines can achieve state-of-the-art (SOTA) results across a wide range of tasks. Specifically, we show that on 35 out of 47 datasets used in prior work (almost 75% of cases), we match or surpass the performance of the current purported SOTA. Strikingly, our baselines often substantially outperform these more sophisticated algorithms. Finally, we correct for the shortcomings highlighted from this prior work by introducing a straightforward standardised methodology for evaluation and by providing our baseline implementations with statistically robust results across several scenarios, useful for comparisons in future work. Our proposal includes simple and sensible steps that are easy to adopt, which in combination with solid baselines and comparative results, could substantially improve the overall rigour of empirical science in offline MARL moving forward.

==> sections/98_checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We are clear in both the Abstract and Introduction about how our paper contributes to Offline MARL research, focusing on the problem of baselines and evaluation protocols. We accurately share the central claims of our paper---that straightforward baselines in offline MARL can achieve SOTA results across many scenarios, which is a result we show with significance later in the paper.}
  \item Did you describe the limitations of your work?
    \answerYes{We have a separate limitations section, with an invitation to the community for further engagement.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{We do not feel that such a section is relevant in the presently nascent field of offline MARL, where we are developing methods to learn optimal control strategies from offline data. Currently, we are still operating in theoretical or hypothetical scenarios, using small-scale, toy-problem simulations.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We have reviewed the ethical guidelines and remain wholeheartedly confident that our contribution does not violate any guideline whatsoever.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Central to this paper is our set of benchmark results, trained using a collection of datasets. Accordingly, we have been pedantic in our reproducibility efforts: we share all baseline code (which achieves SOTA in majority of considered scenarios), along with links to raw experiment data on WandB; we also convert multiple datasets from other authors (at times, very difficult to access!), to a consistent, simple, and stable API format, and make these available publicly, with a guarantee of ongoing maintenance. Instructions for accessing and using this data is also provided in a Google Colab notebook. We further provide an extensive metareview of the field, in the form of another interactive notebook.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All relevant training information is included in the comprehensive appendices.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All experiments were run over 10 seeds, and results are reported with statistical significance tests done. Error bars are included in our main plot, in Figure~\ref{fig:comp_results}. Other plots come from the statistically reliable tools from~\citet{agarwal2022deep} and~\citet{gorsane2022standardised}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{All compute information is provided in the appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{This work leverages datasets from various authors in the literature, and appropriate citations are given in each case.}
  \item Did you mention the license of the assets?
    \answerYes{Details of all the accessed datasets are listed in the appendix, including license information.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We converted datasets from the literature to a consistent and stable API, and these new datasets are available online via a URL. The full methodology for converting the datasets is provided in a Google Colab notebook, also linked in the appendix.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{The license of the various open-source datasets allows us to freely use and repackage the data, and we feel no concerns around consent here.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{This dimension is not applicable to our datasets, since our scenarios deal with fictional, simulated environments, completely separate from anything personally identifiable or offensive.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/_datasets.tex <==
\begin{table}
\centering
\scriptsize
\setstretch{1.5}
\caption{A summary of what datasets key papers in the offline MARL literature used to benchmark their proposed algorithm.} \label{tab:datasets}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c|c}
\textbf{Paper} & \textbf{Source of Datasets} & \textbf{Dataset Labels} & \textbf{Means}, $\mu$ & \textbf{Standard Deviations} \\
\hline

\begin{tabular}{c}
MAICQ% \\ \citep{maicq}
\end{tabular}
&
\begin{tabular}{c}
Self-generated using \\ DOP~\citep{wang2021dop}
\end{tabular}
& \begin{tabular}{c} 
\emph{good} \\
\emph{medium} \\
\emph{poor}
\end{tabular} & \begin{tabular}{c}
$15<\mu<20$ \\
$10<\mu<15$ \\
$0<\mu<10$
\end{tabular} &
\textcolor{xmarkcolour}{Not given}
\\ \hline

\begin{tabular}{c}
MADT% \\ \citep{madt}
\end{tabular}
& 
\begin{tabular}{c}
Self-generated using \\ MAPPO~\citep{yu2022surprising}
\end{tabular}
& \begin{tabular}{c} \emph{replay} \end{tabular} & Given & Given \\
\hline

\begin{tabular}{c}
OMAR% \\ \citep{omar}
\end{tabular}
&
\begin{tabular}{c}
Self-generated using \\ MATD3~\citep{ackermann2019matd3}
\end{tabular}
& \begin{tabular}{c} \emph{replay} \end{tabular} &
\textcolor{xmarkcolour}{Not given} &
\textcolor{xmarkcolour}{Not given} \\
\hline

\begin{tabular}{c}
CFCQL% \\ \citep{cfcql}
\end{tabular}
&
\begin{tabular}{c}
Self-generated using \\ QMIX~\citep{rashid2018qmix}
\end{tabular}
& \begin{tabular}{c}
\emph{medium} \\
\emph{medium-replay} \\
\emph{expert} \\
\emph{mixed}
\end{tabular} &
\textcolor{xmarkcolour}{Not given} &
\textcolor{xmarkcolour}{Not given} \\
\hline

\begin{tabular}{c}
OMAC% \\ \citep{omiga}
\end{tabular}
& Random Subsets from MADT &
\begin{tabular}{c} 
\emph{good} \\
\emph{medium} \\
\emph{poor}
\end{tabular}
& \textcolor{xmarkcolour}{Not given} & \textcolor{xmarkcolour}{Not given} \\ \hline

\begin{tabular}{c}
OMIGA% \\ \citep{omiga}
\end{tabular}
& Random Subsets from MADT &
\begin{tabular}{c} 
\emph{good} \\
\emph{medium} \\
\emph{poor}
\end{tabular}
& Given & \textcolor{xmarkcolour}{Not given} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}\label{tab:datasets}

==> tables/env_scenario_counts.tex <==
% \begin{table}[htbp]
% \centering
% \scriptsize
% \setstretch{1.5}
% \caption{Number of scenarios tested in the papers from the case study.}
% \begin{adjustbox}{max width=0.9\textwidth}
% \begin{tabular}{c|c|c|c|c}
%       & SMAC & MAMuJoCo & MPE & Other \\ \hline
% MAICQ & 4  & --        & --   & --     \\
% MADT  & 21  & --        & --   & --     \\
% OMAR  & 4     & 1        & 3   & --     \\
% CFCQL & 4     & 1        & 3   & --     \\
% OMAC  & 4     & --        & --   & --     \\
% OMIGA & 4     &  3         & --   & --     \\
% \bottomrule
% \end{tabular}
% \label{tab:scenario_counts}
% \end{adjustbox}
% \end{table}


==> tables/macql_maddpg_v_qmix.tex <==
\begin{table}[]
\setstretch{1.5}
\centering
\caption{Three return metrics---the Final, $\langle$Maximum$\rangle$, (Average)---from the two baseline algorithms for each environment, shown across various scenario and dataset quality combinations. Each result is presented with a 95\% confidence interval over 10 seeds. For the Final return, boldface indicates the best performing metric for a given result, and an asterisk (*) indicates a metric is not significantly different from the best performing metric in that situation, based on a heteroscedastic, two-sided t-test with 5\% significance.
}
\vspace{1em}
\label{tab:my-table}
\adjustbox{width=0.5\textwidth}{
\begin{tabular}{cc cc}
\textbf{Scenario} & \textbf{Quality} & \textbf{MADDPG+CQL} & \textbf{QMIX+CQL} \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
8m & Medium &
\RESULT{9.50}{10.75}{11.30}{12.55}{7.98}{0.90} &
\RESULT{0.93}{0.32}{4.15}{1.81}{1.31}{0.14}
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
2s3z & Medium &
\RESULT{6.88}{5.21}{15.42}{2.17}{7.58}{0.56} &
\RESULT{5.03}{2.54}{14.16}{2.05}{9.73}{0.44}
\\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
5m\_vs\_6m & Medium &
\RESULT{3.50}{3.55}{6.17}{0.97}{4.42}{0.32} &
\RESULT{12.04}{3.67}{13.46}{1.96}{7.37}{0.53}
\\ \bottomrule
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{tabular}
}
\end{table}

